Enhancing Prompt Following with Visual Control Through Training-Free Mask-Guided Diffusion

Recently, integrating visual controls into text-to-image~(T2I) models, such as ControlNet method, has received significant attention for finer control capabilities. While various training-free methods make efforts to enhance prompt following in T2I models, the issue with visual control is still rarely studied, especially in the scenario that visual controls are misaligned with text prompts. In this paper, we address the challenge of ``Prompt Following With Visual Control" and propose a training-free approach named Mask-guided Prompt Following (MGPF). Object masks are introduced to distinct aligned and misaligned parts of visual controls and prompts. Meanwhile, a network, dubbed as Masked ControlNet, is designed to utilize these object masks for object generation in the misaligned visual control region. Further, to improve attribute matching, a simple yet efficient loss is designed to align the attention maps of attributes with object regions constrained by ControlNet and object masks. The efficacy and superiority of MGPF are validated through comprehensive quantitative and qualitative experiments.

==> fig_src/maji.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.98\linewidth]{imgs/maji_only.pdf}
  \caption{Qualitative Comparison using majicmixrealistic, we compare our method with baseline model.}
  \label{fig:maji}
  \vspace{-0.2cm}
\end{figure}

==> fig_src/maji_anything.tex <==
\begin{figure*}
  \centering
  \vspace{-3cm}
  %\includegraphics[width=0.9\linewidth]{imgs/other_models_v1.pdf}
   \includegraphics[scale=0.17]{imgs/other_models.pdf}
  \caption{Qualitative Comparison using majicMIX and AnythingV4, we compare our method with baseline model.}
  \vspace{-2cm}
  \label{fig:anything_maji}
  %\vspace{-1.5cm}
\end{figure*}

==> fig_src/steps.tex <==
\begin{figure*}
  \centering
  %\includegraphics[width=1\linewidth]{imgs/Steps.pdf}
  \includegraphics[scale=0.2]{imgs/Steps_v1.pdf}
  \caption{We conduct experiments to explore the impact of altering the number of intervention steps. For consistency, all images are produced using the same random seed.}
  \label{fig:steps}
  \vspace{-0.5cm}
\end{figure*}

==> tables/dataset.tex <==
% \begin{table*}
% \small
% \centering
% \caption{Details about the prompt construction of our benchmark. We list the objects, attributes, and additional descriptions beyond visual controls used to define each prompt in our quantitative evaluations.} 
% %\vspace{-0.2cm}
% \resizebox{0.98\textwidth}{!}{
% \begin{tabular}{l | l | l} 
% \toprule
% \multicolumn{1}{l|}{Category} & \multicolumn{1}{l|}{Entities} & \multicolumn{1}{l|}{ Modifiers} \\
% \midrule
% General & \begin{tabular}{l} backpack, crown, suitcase, chair, balloon, bow, car, bowl, \\ bench, clock, camera, umbrella, guitar, shoe, hat, surfboard, \\ skateboard, bicycle \end{tabular} & \begin{tabular}{l} modern, spotted, wooden, metal, curved, spiky, checkered  \end{tabular} \\
% \midrule
% Fruit & \begin{tabular}{l} apple, tomato, banana, strawberry \end{tabular} & \begin{tabular}{l} sliced, skewered \end{tabular} \\
% \midrule
% Animals & \begin{tabular}{l}cat, dog, bird, bear, lion, horse, elephant, monkey, \\ frog, turtle, rabbit, mouse, panda, zebra, gorilla, penguin \end{tabular} & \begin{tabular}{l} furry, baby, spotted, sleepy \end{tabular} \\
% \bottomrule
% \end{tabular}}
% \label{tb:datasets}
% \end{table*}


\begin{table*}
\small
\centering
\caption{Details about the prompt construction of our benchmark. We list the objects, attributes, and additional descriptions beyond visual controls used to define each prompt in our quantitative evaluations.} 
\vspace{-0.2cm}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l | l} 
%\toprule
%\multicolumn{1}{l|}{Category} & \multicolumn{1}{l|}{Entities} & \multicolumn{1}{l|}{ Modifiers} \\
\midrule
Objects & \begin{tabular}{l} person, bicycle, car, airplane, bus, train, truck, boat, traffic light, fire hydrant, stop sign, parking meter, bench, bird, cat, dog, horse, sheep,\\ cow, elephant, bear, zebra, giraffe, backpack, umbrella, handbag, tie, suitcase, frisbee, skis, snowboard, sports ball, kite, baseball bat, \\
baseball glove, skateboard, surfboard, tennis racket, bottle, wine glass, cup, fork, knife, spoon, bowl, banana, apple, sandwich, orange, \\ broccoli, carrot, hot dog, pizza, donut, cake, chair, couch, potted plant, bed, dining table, toilet, tv, laptop, mouse, remote, keyboard, \\cell phone, microwave, oven, toaster, sink, refrigerator, book,
clock, vase, scissors, teddy bear, hair drier, toothbrush \end{tabular}  \\
\midrule
Attributes & \begin{tabular}{l} red, orange, yellow, green, blue, purple, pink, brown, gray, black, white \end{tabular}  \\
\midrule
Additional Descriptions & \begin{tabular}{l} a bike on a street  \\ a toy on the floor \\  a bench at the beach \\ on the lawn in front of trees \\ next to a tree in the park \\ yellow flowers in a grassy park \\ on the beach near the sea \\ next to a table near the window \\ the light shines through the leaves on the ground \\ next to stacked red gift boxes \\ the huge rocks on the mountaintop \\ on the white floor \end{tabular} \\
\bottomrule
\end{tabular}}
%\vspace{-0.2cm}
\label{tb:datasets}
\end{table*}





==> tables/material.tex <==
\begin{table}[ht!]
  \centering
    \caption{Quantitative Results of baseline and our method on material prompt. We give results under canny. VQA-F, VQA-B, text-text, image-text represent LLM foreground VQA score, LLM background VQA score, clip text similarity between input text prompt and blip captions, clip image-text similrity respectively. Our method achieves best results in all metrics.}
    \label{table:material}
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{c| c c c c |}
  \toprule
  \midrule
  Method & \multicolumn{4}{c|}{Softedge} \\ 
  & VQA-F & VQA-B & text-text & image-text \\
  \midrule
  Baseline & 0.6318 & 0.6048 & 0.4807 & 0.1957 \\
  Baseline(mask) & 0.6239  & 0.5674 & 0.5302  & 0.2684  \\
  Attend & 0.7105  & 0.5942  & 0.5160  & 0.2730  \\
  Structure & 0.5989 & 0.5609  & 0.5277  & 0.2705  \\
  Attr & 0.6580 & 0.6503  & 0.5268  & 0.2760 \\
  Ours & 0.6951 & 0.7293 & 0.4873 & 0.1955 \\
  \midrule
  \bottomrule
  \end{tabular}}
\end{table}

==> tables/one_side_loss.tex <==
\begin{table}
  \centering
    \caption{one side loss}
    \label{table:main}
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{c| c c c c |}
  \toprule
  \midrule
  Method & \multicolumn{4}{c|}{Softedge} \\ 
  & LLM VQA & LLM VQA Background & text-text & image-text \\
  \midrule
  double-side loss & & & & \\
  one-side loss & & & & \\
  \midrule
  \bottomrule
  \end{tabular}}
\end{table}
